Semi-Decentralized Federated Learning with Collaborative Relaying

We present a semi-decentralized federated learning algorithm wherein clients collaborate by relaying their neighbors' local updates to a central parameter server (PS). At every communication round to the PS, each client computes a local consensus of the updates from its neighboring clients and eventually transmits a weighted average of its own update and those of its neighbors to the PS. We appropriately optimize these averaging weights to ensure that the global update at the PS is unbiased and to reduce the variance of the global update at the PS, consequently improving the rate of convergence. Numerical simulations substantiate our theoretical claims and demonstrate settings with intermittent connectivity between the clients and the PS, where our proposed algorithm shows an improved convergence rate and accuracy in comparison with the federated averaging algorithm.

==> system_model_PS.tex <==

% % \documentclass{standalone}
% %  \usepackage{tikz}
% % \usepackage{tikz-3dplot}
% % \usepackage{graphicx}
% % \usetikzlibrary{shapes.multipart}
% % \usetikzlibrary{shapes.symbols}
% % \begin{document}
	
% 	\begin{tikzpicture}[thick,scale=0.5, every node/.style={scale=0.7}]
% 	\node[]  (PS) at(2,5,5) 
% 		{\includegraphics[height = 2.8cm, width = 6cm]{cloud_fig.png}};
% 	\node[inner sep=-2pt]  at(1.8,4.3,5) 	{{\huge  PS}};
	
	
% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c1) at(-12,-6.5,0)
% 	{\includegraphics[scale=0.2]{cell_phone_client.png}}
% 		edge[->,dashed,red] node[below=0.1cm,pos=0.1] {} (PS);
	
% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c2) at(-9.5,-2.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 		edge[-]  (c1)
% 	edge[->,dashed,red]  node[above=0.15cm,pos=0.15] {} (PS);
	
% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c3) at(-7.5,-6.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 	edge[-]  (c1)
% 	edge[->,dashed,red]  node[above=0.1cm,left=0.01cm,pos=0.13] {} (PS);
	
% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c4) at(-4,-4.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 	edge[-]  (c3)
% 	edge[-]  (c2)
% 		edge[->,dashed,red] node[above=0.05cm,left=0.01cm,pos=0.13] {}  (PS);
	
% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c5) at(-2,-7.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 	edge[-]  (c3) edge[->,dashed,red]  node[above=0.15cm,left=0.01cm,pos=0.1] {} (PS);

% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c6) at(0.2,-4,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 	edge[-]  (c4) 
% 	edge[->,dashed,red] node[above=0.15cm,left=0.01cm,pos=0.1] {} (PS);
	

% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c7) at(2.5,-5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 	edge[-]  (c5)
% 	edge[-]  (c6) 
% 	edge[->,dashed,red] node[above=0.1cm,left=0.01cm,pos=0.1] {} (PS);
	

% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c8) at(6,-6.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 	edge[-]  (c5) 
% 	edge[-]  (c7)
% 	edge[->,dashed,red] node[below=0cm,left=0.01cm,pos=0.07] {} (PS);

% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c9) at(11,-7,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 	edge[-]  (c8) 
% 	edge[->,dashed,red] node[above=0.05cm,left=0.01cm,pos=0.1] {} (PS);

% 	\node[inner sep=-2pt,anchor=north,label=below:{}] (c10) at(9.5,-3,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
% 	edge[-]  (c9)
% 	edge[-]  (c7) 
% 	edge[->,dashed,red] node[above=0.2cm,right=0.1cm,pos=0.15] {} (PS);

	
% 	\end{tikzpicture}
% % 	\end{document}

	\begin{tikzpicture}[thick,scale=0.5, every node/.style={scale=0.8}]
	\node[]  (PS) at(2,5,5) 
		{\includegraphics[height = 2.8cm, width = 6cm]{cloud_fig.png}};
	\node[inner sep=-2pt]  at(1.8,4.3,5) 	{{\huge  PS}};
	
	
	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{1}$}] (c1) at(-12,-6.5,0)
	{\includegraphics[scale=0.2]{cell_phone_client.png}}
		edge[->,dashed,red] node[below=0.1cm,pos=0.1] {{\huge $p_1$}} (PS);
	
	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{2}$}] (c2) at(-9.5,-2.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
		edge[-]  (c1)
	edge[->,dashed,red]  node[above=0.15cm,pos=0.15] {{\huge $p_2$}} (PS);
	
	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{3}$}] (c3) at(-7.5,-6.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
	edge[-]  (c1)
	edge[->,dashed,red]  node[above=0.1cm,left=0.01cm,pos=0.13] {{\huge $p_3$}} (PS);
	
	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{4}$}] (c4) at(-4,-4.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
	edge[-]  (c3)
	edge[-]  (c2)
		edge[->,dashed,red] node[above=0.05cm,left=0.01cm,pos=0.13] {{\huge $p_4$}}  (PS);
	
	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{5}$}] (c5) at(-2,-7.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
	edge[-]  (c3) edge[->,dashed,red]  node[above=0.15cm,left=0.01cm,pos=0.1] {{\huge $p_5$}} (PS);

	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{6}$}] (c6) at(0.2,-4,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
	edge[-]  (c4) 
	edge[->,dashed,red] node[above=0.15cm,left=0.01cm,pos=0.1] {{\huge $p_6$}} (PS);
	

	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{7}$}] (c7) at(2.5,-5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
	edge[-]  (c5)
	edge[-]  (c6) 
	edge[->,dashed,red] node[above=0.1cm,right=0.01cm,pos=0.1] {{\huge $p_7$}} (PS);
	

	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{8}$}] (c8) at(6,-6.5,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
	edge[-]  (c5) 
	edge[-]  (c7)
	edge[->,dashed,red] node[below=0cm,left=0.01cm,pos=0.07] {{\huge $p_8$}} (PS);

	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{9}$}] (c9) at(11,-7,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
	edge[-]  (c8) 
	edge[->,dashed,red] node[above=0.05cm,left=0.01cm,pos=0.1] {{\huge $p_9$}} (PS);

	\node[inner sep=-2pt,anchor=north,label=below:{\huge $c_{10}$}] (c10) at(9.5,-3,0) {\includegraphics[scale=0.2]{cell_phone_client.png}}
	edge[-]  (c9)
	edge[-]  (c7) 
	edge[->,dashed,red] node[above=0.2cm,right=0.1cm,pos=0.15] {{\huge $p_{10}$}} (PS);

	
	\end{tikzpicture}
